Parallel Write-Efficient Algorithms and Data Structures for Computational Geometry

In this paper, we design parallel write-efficient geometric algorithms that perform asymptotically fewer writes than standard algorithms for the same problem. This is motivated by emerging non-volatile memory technologies with read performance being close to that of random access memory but writes being significantly more expensive in terms of energy and latency. We design algorithms for planar Delaunay triangulation, $k$-d trees, and static and dynamic augmented trees. Our algorithms are designed in the recently introduced Asymmetric Nested-Parallel Model, which captures the parallel setting in which there is a small symmetric memory where reads and writes are unit cost as well as a large asymmetric memory where writes are $\omega$ times more expensive than reads. In designing these algorithms, we introduce several techniques for obtaining write-efficiency, including DAG tracing, prefix doubling, reconstruction-based rebalancing and $\alpha$-labeling, which we believe will be useful for designing other parallel write-efficient algorithms.

==> aug-bulk.tex <==
\section{Bulk Updates on Augmented Trees}\label{sec:aug-bulk}

One of the benefits of our reconstruction-based approach is that, bulk updates on these augmented trees can be supported directly.
In the case we change the inner trees of interval and range trees as treaps.
For a treap of size $n$ and a bulk update of size $m$, the expected cost of inserting or deleting this bulk is $O(\wcost{}m+m\log(n/m))$ using treaps~\cite{Gu2018}, and the depth is $O(\wcost{}\log m\log n)$ with high probability (\whp{} )~\cite{blelloch2016just,Sun2016PAM,sun2018parallel}.
We note that there are data structures supporting bulk updates in logarithmic expected depth~\cite{blelloch1999pipelining,AS16}, but we are not sure how to make them write-efficient.

Again deletions are trivial.
For interval and range trees, we can just mark all the objects in parallel but apply deletions to inner trees, which requires constant writes per deletion.
For priority tree, we delete can delete points in a top-down manner, using $O((\alpha+\wcost{})\log_\alpha n)$ work per point and $O((\alpha+\wcost{})\log_\alpha^2 n)$ depth.
We now sketch an outline on the bulk insertion.

Assume the bulk size is $m$ and less than $n$ since otherwise we can afford to reconstruct the whole augmented tree.
We first sort the bulk using $O(m\log m+\wcost{}{m})$ work and $O(\wcost\log n)$ depth.
Then we merge the sorted list into the augmented tree recursively, and check each \critical{} node in the tree in a top-down manner.
%Here we assume $\alpha\ge 4$ to guarantee Lemma~\ref{lemma:critical-dynamic}, since in bulk updates, the subtree size.

At any time and for a \critical{} node, we use binary search to decide the new objects inserted in this subtree.
If the overall size of the subtree and the newly added objects overflows $4\alpha^i-2$, we reconstruct the subtree by first flattening the tree nodes, merging with new nodes, rebuilding the subtree using the algorithm in Section~\ref{sec:presort}, and marking the \critical{} nodes in this subtree.
To guarantee Lemma~\ref{lemma:critical-dynamic}, we do not mark the \critical{} nodes with subtree size greater than or equal to $2\alpha^{i+1}-1$.
By doing so, the proof of Lemma~\ref{lemma:critical-dynamic} still holds.
The whole process takes $O(n')$ operations in $O(\wcost{}\log n')$ depth for a subtree with $n'$ nodes.
Note that at least $O(n')$ nodes are inserted between two consecutive reconstructions so that the cost can be amortized.
Otherwise, we just recursively check all the \critical{} children of this node.
Once there are no objects within one subtree, we stop the recursion in this subtree.

Note that the range of a binary search can be limited by the range of the \critical{} parent.
The overall cost for all binary searches is $O(\alpha m \log (n/m))$~\cite{blelloch2016just} (no writes), and the depth is $O(\alpha\log m\log_\alpha n)$.
In summary, the amortize work for merging $m$ new objects in to the tree is $O(\alpha m \log (n/m)+\wcost{}m\log_\alpha n)$, and the depth is $O(\alpha\log m\log_\alpha n+\wcost\log n)$.

We now discuss the bulk updates for the augmented values.
Again for interval trees and range trees, we can just merge all inserted objects into the corresponding inner trees.
Using treaps as the inner trees, merging $m'$ objects to a search tree with $n'$ takes $O(m'\log (n'/m')+\wcost{}m')$ work and $O(\wcost{}\log m'\log n')$ depth.
As a result, for interval and range trees, the work per object in the bulk updates is always no more than the single insertion, and the depth is polylogarithmic for any bulk size.

The bulk update for priority trees is similar to the constructions.
Once there exists an inserted point with higher priority than the root node, we replace root node with this inserted node, and insert the original root node into the corresponding subtree.
Then we leave a hole in the inserted list and recursively apply this process.
This process terminates at the time either the subtree root overflows, we reach a leaf node, or there are more holes than new objects.
The maintenance of augmentations of priority tree takes $O((\alpha+\wcost{})m\log_\alpha n)$ amortized work and $O((\alpha+\wcost{})\log_\alpha^2 n)$ depth.


==> kd-dynamic.tex <==
\section{Dynamic Updates on our \kdtree{s}}\label{sec:kdupdate}

Unlike many other tree structures, we cannot rotate the tree nodes in \kdtree{s} since each tree node represents a subspace instead of just a set of objects.
Deletion is quite simple for \kdtree{}, since we can afford to reconstruct a subtree from scratch when a constant fraction of the objects in the subtree have been removed, and the cost can be amortized.
For insertions, we use a technique called \emph{logarithmic reconstruction}~\cite{overmars1983design}.
It is similar to the binomial heap that at most $\log_2 n$ \kdtree{s} can exist simultaneously with their sizes respecting the power of 2.
Once an object is inserted, we create a \kdtree{} of size one only containing this object.
If there exists a tree with size one already, we flatten them and reconstruct a tree with size two.
This process keeps repeats until there are no trees with the same size.
When querying, we search in all (at most $\log_2 n$) trees.
Using this approach the number of reads and writes on an insertion is $O(\log^2 n)$, and on a deletion is $O(\log n)$. The costs for range queries and ANN queries are $O(n^{(k-1)/k})$ and $O(\log^2 n\cdot O(1/\epsilon)^k)$ respectively, plus the cost for writing the output. %\julian{why is there no $\omega$ term in these work bounds?}

Note that if we apply our write-efficient \batchedshort{p} version when reconstructing the \kdtree{s}, we can reduce the writes (but not reads) by a factor of $O(\log n)$ (i.e.\ $O(\log n)$ and $O(1)$ writes for insertion and deletion).
%(Count size of deletion.) \julian{what about size of deletions?}

When using logarithmic reconstruction, querying up to $O(\log n)$ trees can be inefficient, so here we analyze the bounds when maintaining just a single tree. The query costs are then the same as discussed in Section~\ref{sec:kdconstruct}
The analysis in Section~\ref{sec:kdconstruct} indicates that only the tree height affects the query cost.
To maintain the tree height as $\log_2 n+O(1)$, we can tolerate imbalance between the weights of two subtrees by a factor of $O(1/\log n)$.
Hence, each inserted object contributes $O(\log n)$ amortized writes to all of the nodes on the tree path ($O(\log^2 n)$ reads).
Hence, the amortized work for an insertion is $O(\log^3 n+\wcost{}\log^2 n)$.
For efficient ANN queries, we want the tree height to be $O(\log n)$, which can be guaranteed if the imbalance between two subtree sizes is at most a constant multiplicative factor.
In this case, the amortized work for an insertion is $O(\log^2 n+\wcost{}\log n)$.
%% Remind that using this implementation, we only keep one tree, so the query cost remains the same as the static case discussed in Section~\ref{sec:kdconstruct}, and it is more preferred when queries are significantly more than updates.
%\julian{say the query time} \julian{need $\omega$ in the work bounds}



==> linear.tex <==
\section{LP-type Geometry Problems}\label{sec:lp}

In this section, we study the write-efficient algorithms on several LP-type geometry problems in low-dimensional space.
These problems have linear-work and polylogarithmic-depth randomized incremental algorithms, including linear programming, smallest enclosing disk, and many others~\cite{sharir1992combinatorial}.
Such algorithms have been widely studied in~\cite{Chen2002,Deng1990,Goodrich97,Dyer1995,Ajtai1992,Goodrich1996,Sen95,Alon1994}.  The standard versions of the algorithms require $O(n)$ writes.

In this paper, we introduce a write-efficient version of LP-type algorithms that reduces the number of writes to $O(1)$ while maintaining $O(n)$ reads and polylogarithmic depth.
This version is mainly based on the algorithm in~\cite{blelloch2016parallelism} which provides parallelism and is simple to analyze, and recent work by Har-Peled~\cite{har2016shortest} which only requires constant extra space but is still work-efficient.
%For simplicity we discuss the algorithms in two dimensions, and we can easily apply them to higher dimensions by working out the parameters in the algorithm.
Here we assume $\delta$ is the dimension of the problem.

The key idea in Har-Peled's approach is to simply replace the random
permutation by an arbitrary random sequence that has a uniform
distribution over the constraints (e.g., a hash function).  We can in
parallel generate such a sequence by a standard pseudo-random
generator by Mulmuley~\cite{Mulmuley94}.  The output is uniformly
random on $[n]=\{1,\ldots,n\}$ and $\phi$-wise independent, each
element can be computed in $O(\phi)$ time, and the whole algorithm
uses $O(c'\phi)$ space for an integer constant $c'\ge 12$.  Har-Peled
shows that plugging this sequence into the original algorithms gives
the same asymptotic work bounds.  This is because with probability
less than $1/(20\delta)$ each integer in $[n]$ does not appears in the
first $\bar{c}n$ elements in this sequence for any constant
$\bar{c}\ge 8(5+\lceil \ln \delta\rceil)^2$.  Taking the union bound
shows that the probability that any of the constraints in the final
configuration does not appear is small: $1/20$.
Notice that repeated numbers are not a problem in these algorithms.
At the end of the algorithm, we can verify the solution by testing all
of the constraints, and if a violation is found (with probability no
more than $1/20$), we just restart the algorithms.  Finally, we need
different generators for different recursive levels in the algorithm.
Other details can be found in~\cite{har2016shortest}.

Har-Peled also shows that, as long as $\phi\ge 6\delta+9$, the probability that the $i$'th constraint violates the current configuration is $O(1/i)$.
This not only gives the expected linear work bound, but can be plugged into the analysis by Blelloch et al.~\cite{blelloch2016parallelism} that the length of the longest path in the dependence graph is $O(\log n)$ \whp{}.
As a result, this gives a parallel algorithm with depth $O(\log^{\delta-1}n)$ and the same asymptotic work bound.

Note that in most of these LP-type problems, storing the current configuration only uses constant space ($O(\delta)$ to be more accurate).
Given a \smallmem{} of constant size that can hold the configuration and a constant number of other variables and registers to run such an algorithm, there are no writes required in the whole algorithm (except to write the output). This includes problems like low-dimension linear programming and smallest enclosing disk.
However, there exist special cases like the incremental closest-pair algorithm, which requires linear space to store the configuration.
Here we denote \emph{constant-size LP-type problems} as those requiring constant space ($O(\delta)$ words) to store the configuration.

%In conclusion, given a \smallmem{} with constant size, the algorithm uses expected linear work, $O(\log n)$ depth \whp{}, and no extra writes to generate the final solution.
%The write bound is from the constant space bound, and in total the algorithm requires $\delta$ random number generators each using constant space, and a constant number of other variables and registers to run such an algorithm.

\begin{theorem}
Given $O(\delta^2\log n)$ random bits and a \smallmem{} of constant size, a $\delta$-dimensional constant-size LP-type problem on $n$ objects can be solved in $O(\delta!\,n)$ work, $O(\log^{\delta-1}n)$ depth, and $O(1)$ writes for output on the \anp{} model.
\end{theorem}


==> priority.tex <==
\section{Three-sided Range Query}
In this section we discuss how to address the 3-sided range query as defined in Section \ref{sec:prelim}, with some variant of the priority tree structure (also described in Section \ref{sec:prelim}). Ideally we want work- and write-efficient construction time ($O(n\log n)$ work and $O(n)$ writes), efficient query time (poly-logarithmic) and update time (poly-logarithmic amortized).

\subsection{The Pre-sorted Priority Tree}
With a simple variant of the priority tree we can make the structure write-efficient in construction. We pre-sort all points by their x-coordinates. Then instead of removing the point with the highest priority in each round, we keep it as a dummy point as is, and split the array exactly at the middle of the array (by index). In this case the whole subtree has height at most $2\log n$. The parallel depth and query time is the same with the original priority search tree, and the structure is still static.

\subsection{The Augmented Tree}
We can also answer the query by augmenting a binary search tree with a meldable, persistent heap (on the priority) storing all points in its subtree. This data structure fits the augmented map framework as follows:
\begin{align}
H &= \heap(P, <_Y)\\
M &= \am(X,<_X,Y, H, H.\mb{singleton}, H.\mb{merge}, H.\mb{empty})
\end{align}

\begin{tabular}{@{}r@{ }l@{ }l@{ }l@{ }l}
\hline
Key $K$&: & $X$ & : & the x-coordinate the point\\
Comp. $<_K$&:&$<_X$ &:& compares x-coordinates\\
Value $V$&:&$Y$&: & the Y coordinate\\
AugValue $A$&:&$\heap(P,<_Y)$ &:& a heap of all points, ordered by y\\
Base $g$ &:& $A.\mb{singleton}$ &:& Builds a heap on a single node\\
Combine $f$ &:& $A.\mb{merge}$ &:& Merges two heaps\\
Identity $I$ &:& $A.\mb{empty}$ &:& An empty heap\\
\hline
\end{tabular}

\paragraph{\textbf{Construction.}} We directly use the join-based (bottom-up) construction function in \cite{augmap}. It first sorts all points by their x-coordinates. Then it uses the middle point as the root and recursively builds the left and right subtrees. The subtrees and the root are then connected using \func{join}. The \func{join} function will compute the augmented value of the root by using combine function on the augmented values on its children.
The write-efficient sorting \cite{??} (or the algorithm in Section \ref{alg:incsort}) has $O(n\log n)$ work, linear write and $O(\log n)$ depth. The combine function on a node of subtree size $n$ costs $O(\log n)$. Then the total cost of combine functions according to Lemma \ref{lem:sumlog} should be linear. This means that the extra nodes created is also $O(n)$.

\begin{lemma}[\cite{treearxiv}]
\label{lem:sumlog}
If $T$ is an AVL tree, RB tree, WB tree or treap, $\sum_{T'\subseteq T}\log |T'| = O(|T|)$. Here $T'\subseteq T$ means $T'$ is a subtree rooted at some node in $T$. $|\cdot|$ denotes the size of a tree. This holds on expectation for treaps.
\end{lemma}

Note that when persistence is supported
In all the construction has $O(n\log n)$ work, $O(n)$ space, $O(\log^2 n)$ depth and $O(n)$ writes.

\paragraph{\textbf{Query.}} The query will first search $(x_L,x_R)$ as a range in the outer tree. It finds all related nodes (at most $O(\log n)$) on the outer tree, and pop all points with y-coordinates larger than $y_B$ in the corresponding heaps. Assume that the output size is $k$. The number of all access to heap nodes is no more than $3k$ (all output nodes and their two children). The number of all access to the outer tree is at most $O(\log n)$. Thus the query can be answered in $O(k+\log n)$ work.

\paragraph{\textbf{Update.}} We directly use the insert function on the outer tree, and call the combine function on all nodes on the search path or any node involved in rotations. For any outer balancing schemes this will update or rotate at most $O(\log n)$ nodes in the outer tree. Each update is just two merging of heaps. In total the work is no more than $O(\log^2 n)$.

However note that each update costs work $O(\log^2 n)$, which also means $O(\log^2 n)$ extra space. After $\Omega(n/\log^2 n)$ updates, the total space becomes $\Omega(n)$. If we want to bound the linear space, we can choose to re-build the whole tree after each $O(n/\log^ n)$ updates, giving the amortized cost of $O(\log^3 n)$ work and $O(\log^2 n)$ writes per update.

\subsection{The Priority Tournament Tree}
Here we propose a new data structure addressing the 3-sided range query. This data structure is a hybrid of augmented tree and tournament tree, and thus we call it the \emph{\tournament{}}. This data structure organizes all points in a search tree ordered by the x-coordinate. Then we assign an \augval{} to each tree node top-down, which is the highest priority in its subtree that does not appear as the augmented value in any of its ancestor(s).

\paragraph{\textbf{Construction.}}
The pseudocode of constructing a \tournament{} is shown in Algorithm \ref{alg:tournamentbuild}. We first sort all points in $p$ by x-coordinate (Line \ref{line:tournamentsort}). This is also the order maintained by the tree.
We use the middle point ($p_{n/2}$) as the root (Line \ref{line:tournamentroot}), such that the left and right subtree must be weight-balanced.
Then we find the highest priority $m$ in $p$ and its corresponding index $k$ (Line \ref{line:tournamentmax}). This means that the \augval{} of the root is $m$. We then change the priority of $p_k$ as $-\infty$ (Line \ref{line:tournamentreset}) such that it will never appear as the \augval{} in any lower levels. We then recursively build the left subtree on all points on the left of $p_{n/2}$ and the right subtree on all points on the right (Line \ref{line:tournamentrecursive}). In this process, since we may need to reset the priority to $-\infty$ for some points to guarantee correctness, we copy the priority of each node in advance (Line \ref{line:tournamentcopy}).

In each invocation to \func{FromSorted}, the \func{ParMax} costs $O(n)$ work and $O(\log n)$ depth. All the other work (writes) only has constant cost.
There are in total $\log n$ levels of recursion. In all the construction has $O(n)$ work, $O(n)$ space, $O(\log^2 n)$ depth and $O(n)$ writes.

In the construction process, we can also easily record the location (the tree node) from which each \augval{} comes. This is important to guarantee the efficiency of updates. For simplicity we do not show this process in the code in Algorithm \ref{alg:tournamentbuild}.


\begin{algorithm}[t]
\caption{\func{BuildPTTree}$(A,n)$}
\label{alg:tournamentbuild}
    \SetKwFor{ParForEach}{parallel foreach}{do}{endfch}
\SetKwInOut{Note}{Note}
\Note{Build a \tournament{} in parallel. ``$||$'' means that two recursive calls can run in parallel. The function $\langle m,k\rangle=$\func{ParMax}$(p,f)$ is a parallel function that returns the maximum value in $p$ (according to comparison function $f$) as $m$, and the corresponding index as $k$. \func{Node}$(p)$ returns a new tree node with key $p.x$ and $p.y$.}


\KwIn{An array $p = \{(x_1,y_1),\dots,(x_n,y_n)\}$ of all points ($\in P$).}
\KwOut{The root of the \tournament{} containing all points in $A$.}%
$f(p_1,p_2):(P\times P\mapsto \bool) = (p_1.x<p_2.x)$;\\
$p=$\func{Sort}$(p,f)$\\
\label{line:tournamentsort}
$p'=$ an array of $n$ elements $(x_i,y_i,y'_i)$ of type $P'=X\times Y\times Y$\\
\ParForEach{$(x_i,y_i)\in A$} {
\label{line:tournamentcopy}
$p'[i].x=x_i,p'[i].y=y_i,p'[i].y'=y_i$
}
\Return {\func{FromSorted}$(A)$}\\
  \vspace{.5em}
\SetKwProg{myfunc}{function}{}{}
\myfunc{\func{FromSorted}$(A,0,n)$} {
$f:(P'\times P'\mapsto \bool) = (p_1.y'<p_2.y')$;\\
$\langle m,k\rangle = $ParMax$(A, f)$;\\
\label{line:tournamentmax}
$r=$\func{Node}$(A[n/2])$;\\
\label{line:tournamentroot}
$r.$\func{aug}$=m$; $A[k].y'=-\infty$;\\
\label{line:tournamentreset}
$r.$\func{left}$=$\func{FromSorted}$(A,0,n/2-1)$ $||$ $r.$\func{right}$=$\func{FromSorted}$(A,n/2+1,n)$\\
\label{line:tournamentrecursive}
\Return {$r$}
}
\end{algorithm}


\paragraph{\textbf{Query.}} It is very similar to the augmented-heap version. We search the corresponding range of x-coordinates. For each related subtrees, the augmented values form a heap. We then report all priorities larger than $y_B$.

\begin{figure}
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.8\columnwidth]{figures/rotation.pdf}\\
  \caption{Single rotation illustration.}\label{fig:rotation}
\end{figure}

\paragraph{\textbf{Update.}} We only need to give an algorithm for rotation. One rotation costs $O(\log n)$. We need two functions. One is to pull up an \augval{} of a certain node from its descendants (assigning a new \augval{} to some node). The other is to push the \augval{} of the current node down to one of its descendants (when a node's \augval{} is updated, its original \augval{} may now appear as the \augval{} in some of its descendants). When a rotation occurs, e.g., as shown in Figure \ref{fig:rotation}, there are three steps. First, $B$'s new \augval{} should be directly from $A$'s old \augval{}. In this case $B$'s old \augval{} is now eligible to appear in some lower levels in the subtrees rooted at $E$ or $C$. Thus we push $B$'s \augval{} down. Then we set $B$'s new \augval{} to $A$'s old \augval{} because they represent the same subtree. Finally, now $A$ has new children $D$ and $E$, so it need to pull up a new augmented value from one of its new descendants.

To pull up an \augval{}, we compare the priority in the node itself and the \augval{}s in its two children. If the highest one $m$ is the one from one child, we set the current \augval{} to $m$, and recursively pull up a new \augval{} for this child.
To push down an \augval{} $a$, we go to the branch where the priority comes from, set the corresponding child's \augval{} to be $a$, and recursively push this child's old \augval{} down. Both functions cost $O(\log n)$.

For a weight-balanced tree, the amortized number of rotations per update is constant.  Thus the work (and also the number of writes) of one update to the \tournament{} is $O(\log n)$.

\subsection{Use the $\omega$-way Tree to Save Writes}
The \tournament{} and the augmented tree in this section both can benefit from the technique of using a $\omega$-way tree.


==> tracing.tex <==
\section{DAG Tracing}

\begin{definition}[\ourprob{}]\label{def:probdef}
The \ourprob{} takes as input an element $x$, a directed acyclic graph $G=(V,E)$ that has a specific root vertex $r\in V$ with an in-degree of zero, and a boolean predicate function $f(x,v)$, where $v\in V$.
The \ourprob{} computes the output vertex set $S\subseteq V$ such that $v\in S$ iff $v$ has an out-degree of zero (i.e., it is a leaf) and $f(x,v)$ is true.
\end{definition}

We say that a vertex $v$ is \defn{visible} if $f(x,v)$ is true.

\begin{definition}[\ourprop{}]\label{def:dagproperty}
We say the \ourprob{} has the \ourprop{} when for each visible $v$ except for the root, there is at least one predecessor of $v$ that is visible.
\end{definition}
\begin{center}
\begin{tabular}{cc}
  \toprule
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Variable & Description \\
  $R$ & the set of all visible vertices in $G$ \\
  $D$ & the length of the longest path in $G$ \\
  $S$ & the output set of vertices \\
  \bottomrule
\end{tabular}
\end{center}
\begin{theorem}\label{thm:tracing}
The \ourprob{} can be solved in $O(|R|)$ work, $O(D)$ depth and $O(|S|)$ writes when the problem has the \ourprop{}, each vertex $v\in V$ has a constant in-degree, $f(x,v)$ can be evaluated in constant time, and the \smallmem{} has size $\Omega(D)$.
Here $R$, $D$ and $S$ are defined in the previous table.
%Here $D$ is the length of the longest path in $G$, and $R$ is the set of all visible vertices.
\end{theorem}

\begin{proof}
We first discuss a sequential algorithm using $O(|R|)$ work and
$O(|S|)$ writes.  Because of the \ourprop{}, a naive approach would be
to run a depth-first search (DFS) on to find the visible vertices,
which requires $O(R)$ writes since we need to mark whether a vertex is
visited or not.  However, this approach is not write-efficient when
$|S|=o(|R|)$. We describe a write-efficient solution.

Assume that we have a global ordering $\prec_v$ of the vertices in $G$
(e.g., using the vertex labels) and the DFS is based on this ordering.
Then each vertex $v$ is visited during the search of its predecessor
$u$ that has the highest priority among all visible predecessors of
$v$.  Based on this observation, we do not need to store all visited
vertices.  Instead, when we visit a vertex $v$ via a directed edge $(u,v)$
from $u$, we can check if $u$ has the highest priority among all
visible predecessors of $v$. This indicates whether or not $v$ has been visited before.  As long as we have a \smallmem{} of size $\Omega(D)$ that
keeps the stack of the recursion and each vertex in $V$ has a constant
in-degree, we can find the output set $S$ using $O(|R|)$ work and
$O(|S|)$ writes.  The DFS tree generated by this algorithm
is unique and deterministic, but does not require visiting the vertices
in the exact DFS order.  This key observation can be used to
parallelize the algorithm naturally.

Since the ordering to traverse the vertices can be arbitrary, we can
simply search the DAG in a fork-join manner: we can simultaneously
fork off an independent task for each outgoing edges of the current
vertex, and all of these tasks can be run independently in parallel.
The parallel depth in this case is upper bounded $O(D)$, the depth of
the longest path in the graph.  The bound on the work and number of
writes is the same as the sequential algorithm. We can schedule this
computation either use a work-stealing scheduler or a parallel
depth-first scheduler.
\end{proof}


